GNU epsilon -- an extensible programming language

Reductionism is a viable strategy for designing and implementing practical programming languages, leading to solutions which are easier to extend, experiment with and formally analyze. We formally specify and implement an extensible programming language, based on a minimalistic first-order imperative core language plus strong abstraction mechanisms, reflection and self-modification features. The language can be extended to very high levels: by using Lisp-style macros and code-to-code transforms which automatically rewrite high-level expressions into core forms, we define closures and first-class continuations on top of the core. Non-self-modifying programs can be analyzed and formally reasoned upon, thanks to the language simple semantics. We formally develop a static analysis and prove a soundness property with respect to the dynamic semantics. We develop a parallel garbage collector suitable to multi-core machines to permit efficient execution of parallel programs.

==> indices.tex <==
% -*- mode: latex; fill-column: 79; mode: auto-fill; mode: flyspell; buffer-file-coding-system: utf-8 -*-
\printindex

